In-domain representation learning for remote sensing

Given the importance of remote sensing, surprisingly little attention has been paid to it by the representation learning community. To address it and to establish baselines and a common evaluation protocol in this domain, we provide simplified access to 5 diverse remote sensing datasets in a standardized form. Specifically, we investigate in-domain representation learning to develop generic remote sensing representations and explore which characteristics are important for a dataset to be a good source for remote sensing representation learning. The established baselines achieve state-of-the-art performance on these datasets.

==> figures/relative_plot.tex <==
\begin{figure*}[tb]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \vskip
         \includegraphics[width=1.0\textwidth]{figures/lacc/lacc_ds2}
         \caption{Over datasets}
         \label{fig:lacc_datasets}
     \end{subfigure}~%
     \qquad
     \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \vskip
         \includegraphics[width=1.0\textwidth]{figures/lacc/lacc_sizes2.pdf}
         \vspace*{0.5em}
         \caption{Over sizes}
         \label{fig:lacc_sizes}
     \end{subfigure}
     \qquad
     \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \vskip
         \includegraphics[width=0.7\textwidth]{figures/lacc/labels_lacc.pdf}
         \vspace*{6em}
     \end{subfigure}
    \caption{Aggregated mean relative improvement in logit accuracy of fine-tuning from ImageNet and in-domain representations in comparison to training from scratch.
    % \xiaohua{Maybe showing the same plot with accuracy from Table 3? Accuracy is more intuitive and could also make the plot a bit more dense here (without too much space).}
    % \maxim{sg. I think, going with logit accuracy is more correct when averaging accuracies across wide ranges, but it's less intuitive for now, and it takes a lot of space to describe/discuss, etc. So, will look into only mean accuracies or both.}
    }
    \label{fig:relative-improvement}
\end{figure*}


==> sec_internal.tex <==

\subsubsection{BigEarthNet}
\begin{verbatim}
0: Agro-forestry areas
1: Airports
2: Annual crops associated with permanent crops
3: Bare rock
4: Beaches, dunes, sands
5: Broad-leaved forest
6: Burnt areas
7: Coastal lagoons
8: Complex cultivation patterns
9: Coniferous forest
10: Construction sites
11: Continuous urban fabric
12: Discontinuous urban fabric
13: Dump sites
14: Estuaries
15: Fruit trees and berry plantations
16: Green urban areas
17: Industrial or commercial units
18: Inland marshes
19: Intertidal flats
20: Land principally occupied by agriculture, with significant areas of natural vegetation
21: Mineral extraction sites
22: Mixed forest
23: Moors and heathland
24: Natural grassland
25: Non-irrigated arable land
26: Olive groves
27: Pastures
28: Peatbogs
29: Permanently irrigated land
30: Port areas
31: Rice fields
32: Road and rail networks and associated land
33: Salines
34: Salt marshes
35: Sclerophyllous vegetation
36: Sea and ocean
37: Sparsely vegetated areas
38: Sport and leisure facilities
39: Transitional woodland/shrub
40: Vineyards
41: Water bodies
42: Water courses    
\end{verbatim}

\subsubsection{EuroSat}
\begin{verbatim}
0: AnnualCrop
1: Forest
2: HerbaceousVegetation
3: Highway
4: Industrial
5: Pasture
6: PermanentCrop
7: Residential
8: River
9: SeaLake
\end{verbatim}

\subsubsection{RESISC-45}
\begin{verbatim}
0: airplane
1: airport
2: baseball_diamond
3: basketball_court
4: beach
5: bridge
6: chaparral
7: church
8: circular_farmland
9: cloud
10: commercial_area
11: dense_residential
12: desert
13: forest
14: freeway
15: golf_course
16: ground_track_field
17: harbor
18: industrial_area
19: intersection
20: island
21: lake
22: meadow
23: medium_residential
24: mobile_home_park
25: mountain
26: overpass
27: palace
28: parking_lot
29: railway
30: railway_station
31: rectangular_farmland
32: river
33: roundabout
34: runway
35: sea_ice
36: ship
37: snowberg
38: sparse_residential
39: stadium
40: storage_tank
41: tennis_court
42: terrace
43: thermal_power_station
44: wetland
\end{verbatim}


\subsubsection{So2Sat}
\begin{verbatim}
0: Bare rock or paved
1: Bare soil or sand
2: Bush or scrub
3: Compact high-rise
4: Compact low-rise
5: Compact mid-rise
6: Dense trees
7: Heavy industry
8: Large low-rise
9: Lightweight low-rise
10: Low plants
11: Open high-rise
12: Open low-rise
13: Open mid-rise
14: Scattered trees
15: Sparsely built
16: Water
\end{verbatim}


\subsubsection{UC Merced}
\begin{verbatim}
0: agricultural
1: airplane
2: baseballdiamond
3: beach
4: buildings
5: chaparral
6: denseresidential
7: forest
8: freeway
9: golfcourse
10: harbor
11: intersection
12: mediumresidential
13: mobilehomepark
14: overpass
15: parkinglot
16: river
17: runway
18: sparseresidential
19: storagetanks
20: tenniscourt
\end{verbatim}




\subsection{Internal}
Out of scope for now:
\begin{itemize}
    \item self / semi supervised approaches
    \item what makes a good dataset for representation learning
    \item radar datasets
    \item special processing
    \item model adaptation
\end{itemize}


\section*{Old Introduction}

\begin{verbatim}
Paper story:
1. Consolidate representations learning for remote sensing data.
     - Publish a few representative existing datasets in a common
     format (TFDS).
     - Provide splits to be used with these datasets for enhancing
     future research and reproducibility / comparison.
     - Generate and publish TF-Hub modules for representation
       learning.
     - Present current results
2. Demonstrate in-domain representation learning for small data
   sizes.
     - Compare with common transfer learning approaches, including
     from scratch.
3. Demonstrate diversity in remote sensing data: different
   satellites, resolutions, data types, 
     - In this paper: high-resolution aerial RGB, medium-resolution 
     satellite RGB, medium-resolution multi-spectral imagery.
\end{verbatim}

\todo{
* In-domain representation learning for remote sensing (optical)

* Using a variety of datasets

* Multi-spectral with pre-trained weights

* Datasets/splits and representations available

* Making it available for community

* SOTAs
}


Golden age of remote sensing with the exploding availability of satellite data, many nations working together, ...

Challenges are: a lot of data, efficiency, development, big and important problems to solve... 

Golden age of AI and representation learning for RS data as well. 

Just in 2019 we have seen the release of 3 datasets at unprecedented size for remote sensing classification.

The field is still pretty scattered; individual contributions concentrating on specific problems. Because it's tough and there is only limited infrastructure available.

Difficult to compare past results. Mostly different experiment configurations per paper (eg. 10\%, 20\% or 1000 samples, etc.). We hope to help to contribute to a common problem definition to allow faster iteration of research.

Challenges / applications addressed by remote sensing:
climate change, water security, food security (precision farming/agriculture), disaster prevention (earthquake, landslide forecasting), energy (eg. monitoring power plant usage from space)


Characteristics/specifics of remote sensing data: mostly rotation invariant; often low resolution; reduced diversity; shape often not that relevant; absolute pixel values matter;



Recent comprehensive reviews on deep learning in remote sensing can be found in  \cite{zhu2017:dl_rs_review, cheng2017:resisc45, ball2017:dl-rs-review, zhu2019:dl-rs-review, ma2019:dl-rs-review}.



We want to help to simplify future research (simplifying access to such data by for researchers without background in remote sensing to allow to include remote sensing data in default computer vision and AI research benchmarks/problems).
\begin{itemize}
    \item gathering some common (historically) and newest biggest datasets, and providing them in a standardized form for simpler usage (in TFDS).
    \item publish exact splits (train, validation, test) for these datasets for reproducibility.
    \item provide benchmark results based on these splits using common approaches.
    \item evaluating representation learning approaches in dependence of available data sizes
demonstrating new SOTA performance 
\begin{itemize}
    \item effect of pre-processing
    \item in-domain representation learning vs. ImageNet pre-training
\end{itemize}
\item go beyond common remote sensing RGB imagery - three types of remote sensing data:
\begin{itemize}
    \item high-res RGB 
    \item medium-res RGB
    \item medium-res multi-spectral 
\end{itemize}
    \item publish hub modules for classification and representation feature vectors
\end{itemize}


The main contributions of this paper are:
\begin{enumerate}
    \item Generation and publishing of 5 existing datasets in a standardized format (TFDS). To support reproducibility, we will publish as well a set of train/validation/test splits.
    \item Evaluating remote sensing scene recognition using current state-of-the-art models (training from scratch, transfer learning). Assess the non-trivial effects of data preprocessing and architecture choices.
    \item Demonstrate in-domain representation learning ([potentially] with new SOTA results).
    \item Extend the approaches beyond RGB to all available multi-spectral frequencies.
    \item Publish trained in-domain representations (TF-Hub) modules for improved transfer learning.
\end{enumerate}

% \begin{itemize}
%     \item using training from scratch and transfer learning from ImageNet and in-domain.
%     \item 3 data modes: high-res RGB, med-res RGB, med-res all frequency bands
%     \item architecture, model, preprocessing choices
%     \item effect of in-domain and ImageNet pre-training
%     \item 
% \end{itemize}

\subsubsection{Follow-up work}
\begin{itemize}
    \item Would be great to have a graph show performance correlation on in-domain vs down-stream.
\end{itemize}



\begin{table}[h]
    \centering
    \caption{Accuracy (and logit accuracy) over different training methods and number of used training samples (basic preprocessing). \todo{Move to internal (here only for comparison).}}
    \label{tab:sparse-basic-pp}
    \begin{tabular}{llll}
    \toprule
    {\bf BigEarthNet} &             100 &            1000 &           full \\ 
    
    \midrule
    From scratch   &  14.45\% (-1.78) &  21.41\% (-1.30) &  72.85\% (0.99) \\
    Fine-tune ImageNet     &  17.26\% (-1.57) &  24.55\% (-1.12) & \bf 75.36\% (1.12) \\
    Fine-tune in-domain      &  \bf 18.68\% (-1.47) & \bf 26.85\% (-1.00) &  68.50\% (0.78) \\
    \bottomrule
    \end{tabular}

    \begin{tabular}{llll}
    \toprule
    {\bf EuroSAT} &            100 &           1000 &           full \\
    \midrule
    From scratch   &  60.78\% (0.44) &  85.32\% (1.76) &  96.54\% (3.33) \\
    Fine-tune ImageNet      &  85.25\% (1.75) &  96.04\% (3.19) &  98.92\% (4.51) \\
    Fine-tune in-domain      & \bf 91.33\% (2.35) & \bf 97.04\% (3.49) & \bf 99.13\% (4.73) \\
    \bottomrule
    \end{tabular}

    \begin{tabular}{llll}
    \toprule
    {\bf RESISC-45} &             100 &            1000 &           full \\
    \midrule
    From scratch   &  18.56\% (-1.48) &  43.63\% (-0.26) &  86.47\% (1.85) \\
    Fine-tune ImageNet      &  37.45\% (-0.51) &   78.59\% (1.30) & \bf 95.84\% (3.14) \\
    Fine-tune in-domain      & \bf 43.91\% (-0.24) & \bf 79.36\% (1.35) &  95.31\% (3.01) \\
    \bottomrule
    \end{tabular}

    \begin{tabular}{llll}
    \toprule
    {\bf So2Sat} &             100 &            1000 &           full \\
    \midrule
    From scratch   &  33.98\% (-0.66) &  46.68\% (-0.13) &  62.15\% (0.50) \\
    Fine-tune ImageNet      &  44.85\% (-0.21) &   51.80\% (0.07) &  63.08\% (0.54) \\
    Fine-tune in-domain      & \bf 46.36\% (-0.15) & \bf 52.99\% (0.12) & \bf 63.25\% (0.54) \\
    \bottomrule
    \end{tabular}

    \begin{tabular}{llll}
    \toprule
    {\bf UC Merced} &             100 &           1000 &           full \\
    \midrule
    From scratch   &  45.31\% (-0.19) &  80.47\% (1.42) &  85.16\% (1.75) \\
    Fine-tune ImageNet     &   69.14\% (0.81) &  98.24\% (4.02) &  99.22\% (4.84) \\
    Fine-tune in-domain      &  \bf 91.02\% (2.32) & \bf 99.22\% (4.84) & \bf 99.61\% (5.54) \\
    \bottomrule
    \end{tabular}
\end{table}


==> tables/benchmarks_old.tex <==
\begin{table}[h]
    \centering
    \caption{Results on selected remote sensing datasets. \todo{1000 + Full; reduce size; remove comments columns.}}
    \label{tab:benchmarks}
    \begin{tabular}{lrl}
    \toprule
    Dataset, Reference & Metric and Value &  Comments \\
    
    \midrule
    \bf BigEarthNet & Precision / Recall \\
    \hspace{3mm}\cite{sumbul2019:bigearthnet} & 69.93\% / 77.1\% & S-CNN-RGB (cloud/snow free) \\
    \hspace{3mm}\textit{Ours} & \textit{73.44\% (mAP)} \\
    
    \midrule
    \bf EuroSat & Top-1 \\
    \hspace{3mm}\cite{helber2019:eurosat} & 98.57\% & ResNet-50 fine-tuning ImageNet, val split\\
    \hspace{3mm}\textit{Ours} & \textit{99.20}\% \\

    \midrule
    \bf RESISC-45 & Top-1 \\
    \hspace{3mm}\cite{cheng2017:resisc45} & 90.36\% &  VGG-16 on 20\% train data\\
    \hspace{3mm}\textit{Ours} & \textit{96.83}\% & \\
    
    \midrule
    \bf So2Sat & Top-1 & \\
    \hspace{3mm}\textit{Ours} & \textit{61.02}\% \\
    
    \midrule
    \bf UC Merced & Top-1 \\
    \hspace{3mm}\cite{marmanis2016} & 92.4\% & Overfeat feature extraction \\
    \hspace{3mm}\cite{castelluccio2015} & 97.1\% &  GoogLeNet fine-tuning \\
    \hspace{3mm}\cite{nogueira2016:cnn} & 99.41\%  & 5-fold tuning + SVM \\
    \hspace{3mm}\textit{Ours} & \textit{99.61\%} \\
    
    \bottomrule
    \end{tabular}
\end{table}

==> tables/cross_domain_extended.tex <==
\todo{Missing uc\_merced from scratch}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% n=100
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
    \caption{Accuracy on tasks with 100 examples when using a in-domain representation. FS/ImageNet indicates whether the in-domain representation was trained from scratch or from ImageNet}
    \label{tab:cross-in-domain-100-extended}
    \centering

%% Appendix cross-domain table for n=100
\begin{tabular}{lrrrrr}
\toprule
Source \textbackslash Target & \bigearthnet{} &    \eurosat{} &   \resisc{} &     \sosat{} &  \ucmerced{} \\
\midrule
\imagenet{}               &       17.26 &      85.25 &      37.45 &      44.85 &      69.14 \\
FS                     &       14.45 &      60.78 &      18.56 &      33.98 &      45.31 \\
\bigearthnet{} (FS)       &           - &      84.10 &      28.63 &      44.20 &      58.98 \\
\bigearthnet{} (ImageNet) &           - &      86.87 &      30.86 &      45.29 &      65.23 \\
\eurosat{} (FS)           &       18.16 &          - &      25.72 &      42.53 &      55.86 \\
\eurosat{} (ImageNet)     &       17.85 &          - &      34.90 &  \bf 46.36 &      69.14 \\
\resisc{} (FS)          &   \bf 18.68 &      87.65 &          - &      45.40 &      87.89 \\
\resisc{} (ImageNet)    &       18.26 &  \bf 91.33 &          - &      45.60 &  \bf 91.02 \\
\sosat{} (FS)            &       17.32 &      68.88 &      22.75 &          - &      48.44 \\
\sosat{} (ImageNet)      &       17.31 &      82.11 &      30.05 &          - &      58.98 \\
\ucmerced{} (ImageNet)   &       17.04 &      82.98 &  \bf 43.91 &      44.91 &          - \\
\bottomrule
\end{tabular}

\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% n=1000
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
    \caption{Accuracy on tasks with 1000 examples when using a in-domain representation. FS/ImageNet indicates whether the in-domain representation was trained from scratch or from ImageNet}
    \label{tab:cross-in-domain-1000-extended}
    \centering

%% Appendix cross-domain table for n=1000
\begin{tabular}{lrrrrr}
\toprule
Source \textbackslash Target & \bigearthnet{} &    \eurosat{} &   \resisc{} &     \sosat{} &  \ucmerced{} \\
\midrule
\imagenet{}               &       24.55 &      96.04 &      78.59 &      51.80 &      98.24 \\
FS                     &       21.41 &      85.32 &      43.63 &      46.68 &      80.47 \\
\bigearthnet{} (FS)       &           - &      96.65 &      68.34 &      50.04 &      94.53 \\
\bigearthnet{} (ImageNet) &           - &      96.45 &      67.56 &      50.44 &      94.92 \\
\eurosat{} (FS)           &       24.68 &          - &      56.82 &      50.23 &      92.58 \\
\eurosat{} (ImageNet)     &       25.88 &          - &      71.27 &  \bf 52.99 &      96.09 \\
\resisc{} (FS)          &       26.21 &      96.61 &          - &      51.22 &      97.66 \\
\resisc{} (ImageNet)    &   \bf 26.85 &  \bf 97.04 &          - &      51.98 &  \bf 99.22 \\
\sosat{} (FS)            &       23.45 &      89.86 &      46.13 &          - &      82.42 \\
\sosat{} (ImageNet)      &       24.61 &      94.92 &      66.70 &          - &      94.92 \\
\ucmerced{} (ImageNet)   &       23.17 &      94.96 &  \bf 79.36 &      50.68 &          - \\
\bottomrule
\end{tabular}
    
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% n=full
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
    \caption{Accuracy on the tasks with all training examples when using a in-domain representation. FS/ImageNet indicates whether the in-domain representation was trained from scratch or from ImageNet}
    \label{tab:cross-in-domain-full-extended}
    \centering



%% Appendix cross-domain table for n=None
\begin{tabular}{lrrrrr}
\toprule
Source \textbackslash Target & \bigearthnet{} &    \eurosat{} &   \resisc{} &     \sosat{} &  \ucmerced{} \\
\midrule
\imagenet{}               &   \bf 75.36 &      98.92 &  \bf 95.84 &      63.08 &      99.22 \\
FS                     &       72.85 &      96.54 &      86.47 &      62.15 &      85.16 \\
\bigearthnet{} (FS)       &           - &  \bf 99.13 &      93.21 &      61.90 &      96.88 \\
\bigearthnet{} (ImageNet) &           - &      98.66 &      93.26 &      63.09 &      94.53 \\
\eurosat{} (FS)           &       66.02 &          - &      89.52 &      62.34 &      93.36 \\
\eurosat{} (ImageNet)     &       64.29 &          - &      94.19 &  \bf 63.25 &      97.66 \\
\resisc{} (FS)          &       68.50 &      98.88 &          - &      62.86 &      98.83 \\
\resisc{} (ImageNet)    &       67.20 &      99.05 &          - &  \bf 63.25 &  \bf 99.61 \\
\sosat{} (FS)            &       53.51 &      97.34 &      87.34 &          - &      91.02 \\
\sosat{} (ImageNet)      &       63.07 &      98.70 &      93.96 &          - &      97.27 \\
\ucmerced{} (ImageNet)   &       68.41 &      98.81 &      95.31 &      62.87 &          - \\
\bottomrule
\end{tabular}

\end{table}


==> tables/hparams.tex <==
\todo{} Table with hparams

\begin{table}[h]
    \centering
    \caption{Hyper parameters.}
    \label{tab:hparams}


    \begin{tabular}{ll}
    \toprule
    Name and Values & Comments \\
    \midrule
    
    \multicolumn{2}{l}{\bf Optimizer} \\ 
    \hspace{3mm}SGD & momentum=0.9 \\
    

    \multicolumn{2}{l}{\bf Batch size} \\
    \hspace{3mm}512 & BN virtual batch size=32 \\
    
    \multicolumn{2}{l}{\bf Learning rate} \\
    \hspace{3mm}0.1 and 0.01 & decay 10x per each learning schedule phase $p$\\
    
    \multicolumn{2}{l}{\bf Warmup} \\
    \hspace{3mm}linear & Linear increase of learning rate during the first $w$ steps/epochs\\
    
    
    \multicolumn{2}{l}{\bf Learning schedule} \\
    \hspace{3mm}short & $p={750,1500,2250,2500}$ steps, $w=200$ steps\\
    \hspace{3mm}medium & $p={3000,6000,9000,10000}$ steps, $w=500$ steps\\
    \hspace{3mm}long & $p={30,60,80,90}$ epochs, $w=5$ epochs\\

    \multicolumn{2}{l}{\bf Weight decay} \\
    \hspace{3mm}0.01 and 0.0001 & Important for from scratch\\

    \multicolumn{2}{l}{\bf Decay to init} \\
    \hspace{3mm}\todo{} \\

    \multicolumn{2}{l}{\bf Preprocessing} \\
    \hspace{3mm}\todo{} & \\
    
    \bottomrule
    \end{tabular}
    
\end{table}


==> tables/multichannel.tex <==
\begin{table}[h]
\centering

\todo{} Missing BigEarthNet

\begin{tabular}{l|rrr|rrr}
\toprule
{} & \multicolumn{3}{c}{\eurosat} & \multicolumn{3}{c}{\sosat} \\ 
{} & 100 & 1k & full & 100 & 1k & full \\
\midrule
all &       84.12 &    \bf 96.80 &    \bf 99.36 &  \bf 49.39 &   \bf 55.92 &   \bf 63.64 \\
rgb &   \bf 86.60 &        96.53 &        99.19 &      45.52 &       55.43 &       60.15 \\
\bottomrule
\end{tabular}


\caption{Comparison of using only RGB channels, or all available channels}
\label{tab:multichannel}
\end{table}


